Incremental dimension reduction for efficient and accurate visual anomaly detection

While nowadays visual anomaly detection algorithms use deep neural networks to extract salient features from images, the high dimensionality of extracted features makes it difficult to apply those algorithms to large data with 1000s of images. To address this issue, we present an incremental dimension reduction algorithm to reduce the extracted features. While our algorithm essentially computes truncated singular value decomposition of these features, other than processing all vectors at once, our algorithm groups the vectors into batches. At each batch, our algorithm updates the truncated singular values and vectors that represent all visited vectors, and reduces each batch by its own singular values and vectors so they can be stored in the memory with low overhead. After processing all batches, we re-transform these batch-wise singular vectors to the space spanned by the singular vectors of all features. We show that our algorithm can accelerate the training of state-of-the-art anomaly detection algorithm with close accuracy.

==> sections/sec_incremental_sampling.tex <==
\section{Appendix - Incremental sampling}

While the incremental dimension reduction already can reduce the memory usage by shorten the feature length, we can further reduce the memory usage by reducing the vectors to store in the memory. To achieve this, this appendix presents an algorithm called \emph{incremental sampling}.

\subsection{Algorithm}

The algorithm of incremental sampling is actually sample. Given $N$ vectors, which are divided into batches of $B$ vectors each, we sample the representative one after iterating each batch. Our goal is sampling $r N$ of the $N$ vectors where $r$ is the sampling rate, which is in the range of $[0, 1]$. Given the $b$-th batch, our goal is sampled $bBr$ vectors from the iterated batches so far. This can be achieved by sampling $bBr$ vectors from the previously sampled ones, which have $(b-1)Br$ vectors, and the current batch, which has $B$ vectors, together. The sampling algorithm just follow the original algorithm of PatchCore. In such a case, we reduce the number of vectors to store from $bB$ to $bBr$.

\subsection{Time complexity}

While this algorithm is simple, the analysis of time complexity shows that it actually can reduce the sampling time too. This section analyze the time complexity of incremental sampling, which is based on the number of comparison between a pair of feature vectors. 

First, Equ.~\ref{equ:sampling_time_complexity} shows the time complexity to sample $Nr$ vectors from $N$ without batches:

\begin{equation}
N \times (N \times r) \label{equ:sampling_time_complexity}
\end{equation}
	
\noindent Now we analyze the time complexity by diving the $N$ vectors into batches of $B$ vectors each. Given the $b$-th batch and the $r(b-1)B$ vectors sampled from the previous $b-1$ batches, Equ.~\ref{equ:incremental_sampling_time_complexity} shows the time complexity to sample $rbB$ vectors from the previously sampled ones and the $B$ vectors of the current batch:

\begin{eqnarray}
&  & \sum_{b=1}^{N/B} [B + r(b-1)B][rbB] \nonumber \\
& = & rB^2\sum_{b=1}^{N/B} b + r^2B^2\sum_{b=1}^{N/B} (b-1)b \label{equ:incremental_sampling_time_complexity}
\end{eqnarray}

Equ.~\ref{equ:half_sampling_time_complexity} rewrites the first term in Equ.~\ref{equ:incremental_sampling_time_complexity}, which roughly corresponds to half of the total time complexity in Equ.~\ref{equ:sampling_time_complexity}:

\begin{eqnarray}
&   & rB^2 \sum_{b=1}^{N/B} b \nonumber 
\\
& = & rB^2 \frac{1}{2} \frac{N}{B} (\frac{N}{B} + 1) 
  =   \frac{1}{2} rN (N + B) \label{equ:half_sampling_time_complexity}
\end{eqnarray}

Equ.~\ref{equ:extra_sampling_time_complexity} rewrites the second term in Equ.~\ref{equ:incremental_sampling_time_complexity}:

\begin{eqnarray}
% &   & r^2B^2 \sum_{b=1}^{N/B} (b-1)b 
&   & r^2B^2 (\sum_{b=1}^{N/B} b^2 - \sum_{b=1}^{N/B}b) \nonumber \\
& = & r^2B^2 \frac{1}{6} \frac{N}{B}(\frac{N}{B} + 1)(2\frac{N}{B} + 1) 
  -   r^2B^2 \frac{1}{2} \frac{N}{B}(\frac{N}{B} + 1)   \nonumber \\
& = & r^2 \frac{1}{6} \frac{N(N + B)(2N + B)}{B} 
  -   r^2 \frac{1}{2} N(N + B)   \label{equ:extra_sampling_time_complexity}
\end{eqnarray}

\noindent While the second term is more complicated than Equ.~\ref{equ:half_sampling_time_complexity}, if $B$ is chosen such that $B/N$ is close to $r$, the first term in Equ.~\ref{equ:extra_sampling_time_complexity} will be close to $rN^2/3$, namely, one third of the total complexity. By combining with the time complexity in Equ.~\ref{equ:half_sampling_time_complexity}, the time complexity of incremental sampling will be $1/2 + 1/3=5/6$ times $rN^2$, meaning that it can reduce 1/6 of the time complexity. 

It should be noted that before sampling, we need to transform all vectors based on the latest $U^{1,b}$ and $S^{1,b}$. While the transformation requires extra computation time, because it only involved the sampled ones, not all visited vectors, it will be still efficient. 

One parameter of incremental sampling controls when to trigger the resampling. While we can resample after transforming every batch, we can also defer the sampling till more vectors are collected. We can such a scheme \emph{buffering}. Our experiment shows that when block size is small, buffering can trade off between memory usage and the sampling speed. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[!tb]
	\centering
	\caption{
		Benchmark of time and memory complexity on \emph{hazelnut} of MVTec AD with incremental sampling. 
	}
	\label{table:time_space_incremental_sampling}
	\begin{tabular}{cccc|cc}
		& $k$
		& $B$
		& \makecell{Buffering}
		& \makecell{Memory\\(MiB)}
		& \makecell{Time\\(seconds)}
		\\
		\hline
		& N/A
		& N/A
		& N/A
		& 8719
		& 35307
		\\
		& 128
		& 32K
		& All
		& 4260
		& 5776
		\\
		& 128
		& 32K
		& No
		& 3189
		& 3962
		\\
		& 128
		& 16K
		& No
		& 2660
		& 4413
		\\
		& 128
		& 8K
		& No
		& 2267
		& 6119
		\\
		& 128
		& 32K
		& $3\times$
		& 3318
		& 4568
		\\
		& 128
		& 16K
		& $3\times$
		& 2808
		& 4475
		\\
		& 128
		& 8K
		& $3\times$
		& 2417
		& 3907
		\\
	\end{tabular}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Experiments}

To benchmark incremental sampling, we use WideResnet50~\cite{:/conf/bmvc/2016/zagoruyko_wrn} as the feature extraction model, and follow the same way of feature extraction in Section~\ref{sec:experiment}. In this section, $k$ is the number of dimensions to reduce, where N/A means that reduction is disabled. $B$ is the number of vectors per batch. In the column \emph{Buffering}, \emph{All} means that all vectors are buffered, implying that incremental sampling is disabled. \emph{No} means that no vectors are buffered, implying that incremental sampling is applied on every batch. $3\times$ means that incremental sampling is applied once $3$ times the targeted number of vectors are buffered.

Table~\ref{table:time_space_incremental_sampling} lists the computation time and maximal memory usages when training on the class $hazelnut$ of MVTec AD. Here we set the batch size to 1 in order to minimize the memory usage of feature extraction, and used 1 CPU core only so there is no parallelism in the calculation. Note that here we implemented the sampling in numpy, as we found that these functions in torch might cause unstable memory usages. 

While our incremental dimension reduction algorithm already reduced the memory usage from 8.7GB to 4.3GB, with incremental sampling, the memory usage could be further reduced to 3.2 - 3.3GB. When using smaller $B$, we can further reduce the memory usage, but the sampling time can increase. For instance, by setting $B=8K$, the memory usage was reduced to 2267 MiB, but the sampling time increased to 6119 seconds. When using buffering ($3\times$), the memory usage is slightly increased than that without buffering, but the sampling time is reduced.

Tables~\ref{table:incremental_sampling_image_auroc} and ~\ref{table:incremental_sampling_pixel_auroc} list the image-wise and pixel-wise AUROC, respectively, on MVTec AD. It can be seen that incremental sampling lead to almost identical accuracies on categories of objects, and small difference on the categories of textures. Meanwhile, buffering shows almost no differences in accuracies.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[!tb]
	\caption{
Image AUROC (\%) on MVTec AD with incremental sampling. 
}
	\label{table:incremental_sampling_image_auroc}
	\centering
	% \setlength\tabcolsep{2.5pt} % default value: 6pt
	\begin{tabular}{ll|rrrr}
& $k$ & N/A & 128 & 128 & 128 \\
& $B$ & N/A & 32K & 32K & 32K \\
& Buffering & N/A & All & No & $3\times$ \\
\hline
& Average & 99.0 & 98.9 & 98.9 & 98.9 \\
& Texture & 99.3 & 99.0 & 98.9 & 98.9 \\
& Object & 98.9 & 98.9 & 98.9 & 98.9 \\
\hline
& carpet & 99.2 & 98.1 & 98.0 & 98.0 \\
& grid & 99.3 & 99.2 & 99.0 & 99.1 \\
& leather & 100.0 & 100.0 & 100.0 & 100.0 \\
& tile & 99.1 & 99.2 & 99.1 & 99.1 \\
& wood & 98.9 & 98.4 & 98.3 & 98.3 \\
\hline
& bottle & 100.0 & 100.0 & 100.0 & 100.0 \\
& cable & 99.7 & 100.0 & 100.0 & 100.0 \\
& capsule & 96.2 & 96.2 & 96.4 & 96.1 \\
& hazelnut & 100.0 & 100.0 & 100.0 & 100.0 \\
& metal nut & 99.9 & 99.9 & 99.9 & 99.8 \\
& pill & 95.2 & 95.1 & 95.2 & 95.7 \\
& screw & 98.5 & 97.9 & 98.2 & 98.2 \\
& toothbrush & 100.0 & 100.0 & 99.4 & 99.4 \\
& transistor & 100.0 & 100.0 & 100.0 & 100.0 \\
& zipper & 99.3 & 99.6 & 99.6 & 99.5 \\
	\end{tabular}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[!tb]
	\caption{
Pixel AUROC (\%) on MVTec AD with incremental sampling. 
}
	\label{table:incremental_sampling_pixel_auroc}
	\centering
	% \setlength\tabcolsep{2.5pt} % default value: 6pt
	\begin{tabular}{ll|rrrr}
& $k$ & N/A & 128 & 128  & 128  \\
& $B$ & N/A & 32K & 32K & 32K \\
& Buffering & N/A & All & No & $3\times$ \\
\hline
& Average & 97.9 & 97.9 & 97.8 & 97.8 \\
& Texture & 97.3 & 97.3 & 97.3 & 97.3 \\
& Object & 98.2 & 98.1 & 98.1 & 98.1 \\
\hline
& carpet & 98.9 & 99.1 & 99.1 & 99.0 \\
& grid & 98.1 & 97.9 & 97.8 & 97.8 \\
& leather & 99.1 & 99.3 & 99.3 & 99.3 \\
& tile & 95.6 & 95.0 & 95.0 & 95.0 \\
& wood & 94.6 & 95.2 & 95.2 & 95.2 \\
\hline
& bottle & 98.3 & 98.4 & 98.4 & 98.4 \\
& cable & 98.3 & 98.7 & 98.7 & 98.7 \\
& capsule & 98.7 & 98.7 & 98.7 & 98.7 \\
& hazelnut & 98.5 & 98.6 & 98.6 & 98.6 \\
& metal nut & 98.4 & 98.2 & 98.3 & 98.2 \\
& pill & 96.9 & 95.3 & 95.2 & 95.3 \\
& screw & 99.2 & 99.0 & 99.0 & 99.0 \\
& toothbrush & 98.8 & 98.7 & 98.7 & 98.7 \\
& transistor & 96.7 & 96.9 & 96.9 & 96.9 \\
& zipper & 98.7 & 98.8 & 98.8 & 98.8 \\
	\end{tabular}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Summary}

Besides incremental dimension reduction, this appendix presents incremental sampling, another technique to make PatchCore efficient. Incremental sampling not only reduces the vectors to store in the memory, but also accelerate the sampling. By combining both incremental schemes together, we can further reduce the memory footprint required by PatchCore.



